Accurate photometric redshift probability density estimation - method comparison and application

We introduce an ordinal classification algorithm for photometric redshift estimation, which significantly improves the reconstruction of photometric redshift probability density functions (PDFs) for individual galaxies and galaxy samples. As a use case we apply our method to CFHTLS galaxies. The ordinal classification algorithm treats distinct redshift bins as ordered values, which improves the quality of photometric redshift PDFs, compared with non-ordinal classification architectures. We also propose a new single value point estimate of the galaxy redshift, that can be used to estimate the full redshift PDF of a galaxy sample. This method is competitive in terms of accuracy with contemporary algorithms, which stack the full redshift PDFs of all galaxies in the sample, but requires orders of magnitudes less storage space. The methods described in this paper greatly improve the log-likelihood of individual object redshift PDFs, when compared with a popular Neural Network code (ANNz). In our use case, this improvement reaches 50\% for high redshift objects ($z \geq 0.75$). We show that using these more accurate photometric redshift PDFs will lead to a reduction in the systematic biases by up to a factor of four, when compared with less accurate PDFs obtained from commonly used methods. The cosmological analyses we examine and find improvement upon are the following: gravitational lensing cluster mass estimates, modelling of angular correlation functions, and modelling of cosmic shear correlation functions.

==> prediction_interval_estimation.tex <==
\begin{itemize}
 \item Say that I compare ordinal class conditional estimator, Quantile Regression Neural Networks and Quantile Regression Forests 
 \item Give results with respect to Ramp loss and Pinball loss, tuning steps into appendix
 \item Discuss consequences 
\end{itemize}


==> trash.tex <==
%\\
%The performance of the stacked probability density function $p(z)$, denoted as SMNLL, can be quantified analogously as
%\begin{equation}
%	SMNLL = -\frac{1}{N} \sum_{i = 1}^{N} \log{\left(\hat{p}(z_i)\right)} \, .
%	\label{eq:snlp}
%\end{equation}
%A common alternative to the Kullback-Leibler divergence is the integrated squared error (ISE) \citep{Sugiyama2010, Fan2004, Scott1991}, but it is computationally more expensive to evaluate \citep{Holmes2012} and will therefore not be considered in this work.
%\\
%The KS statistic commonly used in astrophysics \citep{bonnet, tpz, dessanchez}
%\begin{equation}
%	KS = \underset{z}{\text{max}} | F(z) - \hat{F}(z) | \, ,
%\end{equation}
%is not appropriate for the direct evaluation of photometric redshift cond. PDF or stacked redshift PDF estimates. The KS statistic is useful to test whether a sample of photometric redshift point predictions is drawn from the same distribution as the spectroscopic redshift values. 
%However here we compare estimates of probability density functions and not point estimates, therefore we use the MNLL and SMNLL.


The accurate estimation of redshift probability density functions (pdfs) from samples of photometrically observed objects will be vital in order to effectively use future large area photometric surveys like the Dark Energy Survey or Euclid for cosmology. We extend classification based pdf estimation by using a classifier that correctly treats redshift bins as ordered quantities. Incorporating this additional information improves the average log likelihood of the spectroscopic redshifts given the redshift probability density function estimates for each object at the 15\% level. We adapt the smoothing of the density estimate for each object individually, which improves the average log likelihood at the 13\% level. To efficiently tackle large photometric datasets, we develop a storage efficient parametrization for the objects redshift probability density function. This enables us to express the object's redshift probability density functions using on average $5$ to $6$ values while maintaining the same overall accuracy compared to contemporary algorithms. We demonstrate the quality of the proposed algorithms using a subsample from the CFHTLS Wide survey. To compare our algorithms with a popular Neural Network code we estimate the inverse critical surface density of a gravitational lens with a fixed redshift marginalized over the redshift distribution of background sources. The estimates obtained using the Neural Network differ from the true (spectroscopic) value up to 12.8\% for high redshift lenses. Using the methods described in this work we can obtain an error of only 0.5\%.\footnote{A software package implementing all discussed algorithms will be available on the first authors homepage.}

\subsubsection{Weighting the Catalogue}
As can be seen from Figure (\ref{zspec_plot}), the spectra from the VIPERS survey introduce a very artificial redshift distribution and contain a large number of luminous red galaxies (LRGs), which makes our dataset not a very realistic dataset for weak lensing analyses. 
\\
In order to probe whether the result changes, if we make the catalogue more realistic, we remove the VIPERS spectra from the original catalogue and reweight the magnitude-redshift distribution. For the new distribution we use the analytical model specified in \citet{Lima2008} for the i band magnitude $p(i)$ and the conditional spectroscopic redshift distribution $p(z | i)$ of a realistic DES Mock catalogue
\begin{equation}
	p(i) = A \exp{\left[\left(\frac{i - 20}{0.29}\right)^{0.5}\right]} \, ,
	\label{eq:model_i}
\end{equation} 
\begin{equation}
	p(z | i) = B z^2 \exp{\left[- \left(\frac{z - (b_1 + b_2 (i - 20) + b_3 (i - 20)^2}{c_{1} + c_{2} (i - 20)^{c_3}} \right)^2\right]} \, ,
	\label{eq:model_cond_pdf}
\end{equation}
where $A$ and $B$ are constants fixed after normalizing the distributions to unity over $z \in [0, 1.5]$ and $i \in [20, 24.5]$ respectively. We use the model parameters from \citet{Lima2008} $(b_1, b_2, b_3, c_1, c_2, c_3) = (-0.2, 0.75, -0.28, 0.39, 0.012, 3.2)$.
Since our goal is to change the spectroscopic redshift distribution of our catalogue, we retrain the methods in order to avoid sample selection bias \citep{Heckman1979}, which will arise since the training set applied previously will no longer be representative for the magnitude-redshift distribution of our reweighted catalogue. Retraining our methods using weighted data is difficult, since we would need to include these weights into our algorithms. We therefore propose an alternative based on the empirical probabiliy density function \citep{Scott1991} defined in the one-dimensional case for a sample containing N objects as
\begin{equation}
 \hat{p}(x) = \frac{1}{N} \sum_{i = 1}^{N} \delta(x - x_i)
 \label{eq:emp_pdf}
\end{equation} 
where $\delta$ is the delta distribution and $x_i$ are the values in our dataset.
Weighting $\hat{p}(x)$ with respect to $f(x)$ can be achieved by introducing a weighting function $w(x)$ as
\begin{equation}
	\hat{f}(x) = A \,  w(x) \,  \hat{p}(x)
\end{equation}
where A is a normalization factor. Using equation (\ref{eq:emp_pdf}) we can rewrite this as
\begin{equation}
 \hat{f}(x) = \frac{1}{\sum_{i = 1}^{N} w(x_i)} \sum_{i = 1}^{N} w(x_i) \delta(x - x_i) \, .
\end{equation} 
From this equation we see that the weights $w(x_i)$ are just the values of $f(x)$ evaluated at the data points $x_i$ from the original sample such that the reweighed empirical probability density function now reads
\begin{equation}
	\hat{f}(x) = \frac{1}{\sum_{i = 1}^{N} f(x_i)} \sum_{i = 1}^{N} f(x_i) \delta(x - x_i) \, .
 \label{eq:emp_pdf_re}
\end{equation}
Sampling from the distribution defined in equation (\ref{eq:emp_pdf_re}) is equivalent to drawing weighted bootstrap samples. We calculate the weights for each object in our sample from the model distributions (Eqn. \ref{eq:model_i}, Eqn. \ref{eq:model_cond_pdf}) and draw weighted boostrap samples of the same size as the original catalogue. Figure \ref{weighting_distri} compares the spectroscopic redshift distribution and the distribution in the \textit{i}-band between the original and the reweighted catalogue. 
%\begin{figure}
%   \centering
% \includegraphics[scale=0.4]{./insert_plots/weighted_distribution.pdf}
%   \caption{ \label{weighting_distri} Effect of the weighting scheme on the redshift and i band magnitude distribution of the original CFHTLS-Wide survey catalogue.  } 
%\end{figure}
Figure \ref{comparison_sigcrit_weight} compares the MWL estimates obtained using the HWE element, which was considered the most efficient algorithm in the previous section, the point estimate from ANNz, and the spectroscopic redshift values.
%\begin{figure}
%   \centering
% \includegraphics[scale=0.4]{./insert_plots/sig_crit_comparison_reweighted.pdf}
%   \caption{ \label{comparison_sigcrit_weight} Comparison of the MWL metric calculated using the stacked redshift %distributions estimated using the ANNz and HWE algorithms. We use a reweighted test set from the CFHTLS Wide dataset (see text).  } 
%\end{figure}
Following Section (\ref{eq:testingframe}), we split the reweighted dataset into a training set, a validation set and a test set containing $(7700 , 2699, 3076)$ objects respectively. Figure \ref{comparison_sigcrit_weight} shows a very similar result to the one obtained in the previous section, indicating that accurate estimation of the stacked redshift distribution is mainly important for high lens redshifts.

%Table \ref{cap:algo_comp} compares the performance of the QRF, NOCP and OCP algorithm with respect to the SNLP loss for the whole redshift range and in the three redshift bins ($[0, 0.585[$, $[0.585, 0.7488[$ and $[0.7488, 3.818[$) obtained by equal frequency binning. The Benchmark for the SNLP loss is a Kernel estimator (Eqn. \ref{eq:kern_dens_def}) applied to the spectroscopic data in the Test set and respective bins. The bandwidth is selected from the standard Scotts rule (Eqn. \ref{eq:bw_select_scott} with $a = 1.06$). 
%\\
%The SNLP loss for all three algorithms is approximately equal, indicating that the stacking process reduces the variance of the single object conditional pdfs. This can also be seen in the three bins where we stacked the single object pdfs by weighting the respective redshift bins (Eqn. \ref{eq:stack_single_pdf}), cutting out the probability tail outside and renormalizing the result. Here we see that the stacked estimate shows superior performance compared with the unconditional estimator obtained from the spectroscopic redshift of the objects in the respective bin. We note however that the Scotts rule assumes a Normal reference density (or close to normal), which will not be the case when applied to the single redshift bins. Therefore we can assume that the selected bandwidth is not optimal for the unconditional kernel estimator, resulting in inferior performance compared with the stacked conditional pdfs that use a locally selected bandwidth for the conditional pdf of each object. 
%We also add a small threshold of -0.0000001 noch was zu log likelihood, log is natural logarithm
%Benchmark Scott rule, Gauß Kernel on test[,1]: SNLP = -0.110
%However will depend on the Samplesize !!!!
%Figure \ref{comparison_distri} plots the resulting estimates for the stacked redshift pdf for each algorithm. We see that the pdfs are very similar and the slight differences will most likely not affect follow up analysis. We note that the result for the QRF algorithm is slightly undersmoothed (the bandwidth is too low) resulting in spurious bumps around the peak. This effect can be easily corrected for by picking a slightly larger bandwidth as is the case for the OCP and NOCP algorithms. To demonstrate that using a global bandwidth is in general sufficient to obtain good estimates for the stacked pdf we stack the QRF weights according to equation \ref{eq:equalweights} and select the bandwidth according to equation \ref{eq:bw_select_scott} with $a = 1$, which shows great consistency with the stacked pdf obtained from the OCP algorithm. 

%\begin{table}
%\begin{center}
%  \begin{tabular}{ c | c | c | c |} 
%         & QRF & NOCP & OCP \\ \hline
%Hjort BW & -0.1073    & -0.1052     & -0.1067    \\ 
%Scott BW &  -0.1061   & -0.1036     & -0.1056 \\  
%\\\hline
%  \end{tabular}
%\caption{\label{cap:algo_comp} Comparison of Quantile Regression Forest (QRF), ordinal classification pdf estimator %(OCP) and nonordinal classification pdf estimator (NOCP) for global stacking measured by the mean negative log %likelihood.  }
%\end{center}
%\end{table}



%Importance of BW selection: 
%OCP: min = -1.27      max = -0.71
%einfach die CV ergebnisse verwenden um die wichtigkeit zu unterstreichen



%\begin{table}
%\begin{center}
%  \begin{tabular}{ c | c | c  } 
%BW mod	    & Scott BW    & Hjort BW   \\ \hline\hline
%0.7         & -1.16       & -0.97       \\ 
%0.8         & -1.19       & -1.03        \\ 
%0.9         & -1.22       & -1.08       \\
%1.0         & -1.24       & -1.12       \\
%1.1         & -1.26       & -1.15       \\
%1.2         & -1.27       & -1.17       \\
%1.3         & -1.27       & -1.19      \\
%\\
% \end{tabular}
%\caption{\label{cap:bw_dependency} MNLP scores for the best performing setup of the OCP algorithm on the selected bandwidth as obtained on the validation set. The Gaussian kernel is used. The variations with respect to all parameters (Tab. \ref{tab:model_select_pdf_comparison}) is larger and at the 44\% level.}
%\end{center}
%\end{table}




We see from figure (\ref{comparison_distri}) that all discussed algorithms are able to accurately estimate the overall spectroscopic redshift distribution of the sample. The HWE, being a point estimate, does not estimate the cond. PDF. If the cond. PDF for single point objects is explicitly required, we can do this very efficient using the OCP-GMM method which requires a storage capacity of 5 to 6 floating point numbers per object on average.
\\
In the following we compare the performance of the different methods of estimating the stacked photometric redshift PDF in more detail. 
%HWE ähnlich 1NN ... besser??? keine ahnung
%Discussion einfügen!!!

The QRF, NOCP and OCP algorithms perform similarly (Tab. \ref{cap:algo_comp}) both in terms of their global accuracy as measured by the SMNLP loss and their local accuracy measured in the three different bins. Since the bandwidth selected by the cross-validation scheme (\S \ref{subsec:bandwidth_select}) for the QRF algorithm is slightly lower than for OCP and NOCP (Tab. \ref{tab:model_select_pdf_comparison}), the estimated PDF shows features around the peak of the distribution (Fig. \ref{comparison_distri}). Selecting a different bandwidth, for instance a global bandwidth (Eqn. \ref{eq:equalweights}) selected using Scotts rule, removes these features. We see that the quality of the estimate in the central bin is best and degrades in the tails, which is expected due to the decreasing data density. The stacked PDFs outperform the HWE slightly in the bins, indicating that stacking photometric redshift cond. PDFs has advantages over using the HWE in combination with a kernel density estimate and a bandwidth selected using Scotts rule. 
\\
OCP-GMM shows solid overall performance on par with the contemporary algorithms. The strength and weaknesses are however distributed differently across the bins compared with the QRF, OCP and NOCP algorithms. This is likely due to the fact that the OCP-GMM does not base its estimate on kernel centres like QRF and OCP, but instead fits the Gaussian mixture model to the weighted data. In contrast, QRF and OCP perform similarly since they are both obtained by a weighted kernel density estimate on the spectroscopic training data (Eqn. \ref{eq:cond_prob}). The inferior result obtained with the kernel estimator applied to the spectroscopic redshifts of the test set objects in the three bins can be explained by noting that the bandwidth for this estimator was selected using Scotts rule, which assumes a normal reference density. This assumption will not be met in the bins. For QRF, OCP, NOCP, OCP-GMM and HWE, we made explicit use of the fact that we estimate the redshift distribution in a certain redshift bin by cutting the estimated PDF at the bin edges. The kernel estimator obtained from the spectroscopic values in this bin does not use this information and will attribute a nonzero probability to values outside that bin, degrading the SNLP loss. 


%\begin{figure}
%   \centering
% \includegraphics[scale=0.4]{./plot_distris_binning/ScatterPlot.pdf}
%   \caption{ \label{scatterplot_weight} Scatterplot of intrinsic size (\S \ref{eq:intrins_size}) against the %magnitude in the $i$ Band of the CFHTLS survey for a respective random subsample of 10000 objects. We plot the %corresponding distribution of the spectrophotometric dataset and the shear catalogue.  } 
%\end{figure}



\subsection{Model Tuning}
\label{sec:mod_tune}
We tune the Quantile Regression Forest (QRF) and the classification based PDF estimators (OCP and NOCP) using two disjunct datasets, the training and validation set, as detailed in section (\ref{sec:mod_tune}). The estimators for the conditional PDF (Eqn. \ref{eq:cond_prob}) are evaluated with respect to the mean negative log likelihood loss (Eqn. \ref{eq:mnlp}). During cross validation we search for the combination of parameters listed in Table \ref{tab:model_select_pdf_comparison} which gives rise to the lowest loss. In this process we adapt the bandwidth selection as described in Section \ref{subsec:bandwidth_select}. The maximum number of components in the Gaussian Mixture Model used as part of the OCP-GMM estimator (\S \ref{subsec:fit_gmm}) was selected analogously.   
\\
We note that the proposed bandwidth selection procedure improves the quality of the cond. PDF estimate compared with the estimates obtained by applying the bandwidth selection rule used in \citet{Frank2009}. The OCP algorithm applied with the cross validated bandwidth selection scheme (${\rm MNLL} = -1.27$) improves upon the method used in \citet{Frank2009} (${\rm MNLL} = -1.12$) at the 13\% level as measured on the validation set. The test set error (${\rm MNLL} = -1.26$) is very similar to this value implying that the performance gains obtained by picking a bandwidth on the validation set propagates into the final test error. 
%Ich hab mal irgendwo gelesen, das log likelihood irgendwie undersmoothed
%\begin{table}
%\centering
%\begin{tabular}{|c||c|c|}
%   Tuning parameters  & QRF method            & OCP/NOCP method     \\\hline\hline
%nodesize              & 1, 5, \textbf{7}      & \textbf{1}, 3     \\
%mtry                  & \textbf{5}            & 2, \textbf{5}     \\
%BW                    & \textbf{Scott}/Hjort  & \textbf{Scott}/Hjort \\
%BW mod                & 0.7, \textbf{0.8} ... 1.3    & 0.7 ... \textbf{1.3}    \\
%Kernel                & g, e, \textbf{t}      & \textbf{g}, e, t 
%\end{tabular}
%\caption[Tuning parameters comparison cond. pdf]{Model parameters of the Quantile Regression Forest (QRF) and the classification based PDF estimation algorithms (OCP/NOCP) selected during Cross-Validation. 'nodesize' and 'mtry' are model parameters of the Random Forest described in Section (\ref{algorithms}). 'BW' denotes the bandwidth selection rules. The 'Hjort'/'Scott' rules are defined in Equations \ref{eq:bw_select_hjort}/\ref{eq:bw_select_scott}) respectively. 'BW mod' denotes the bandwidth modification factor employed in the bandwidth selection rules (Eqn. \ref{eq:bw_select_hjort}, Eqn. \ref{eq:bw_select_scott}). 'g', 'e', 't'  symbolize the Gaussian, Epanechnikov and triangular kernel functions \citep[][page 140]{Scott1991}. The best parameter configuration for each algorithm is marked in bold type.}
%\label{tab:model_select_pdf_comparison}
%\end{table}

%\\
%The discussion focusses on three main points. Treating the binned redshift as an ordinal attribute as done in the OCP and OCP-GMM algorithms improves the quality of the estimated cond. PDFs. The stacked photometric redshift distribution can be accurately estimated with a single floating point number, the highest weight element (\S \ref{subsec:hwe}).

%\begin{table}
%\begin{center}
%  \begin{tabular}{ c | c | c | c | c | c  } 
%	     & QRF    & NOCP   &   OCP   & HWE & GMM  \\ \hline\hline
%SMNLL    & -0.1137  & -0.1093  & -0.1119   & -0.1097    & -0.1053    \\ 
%B1       & -1.0052  & -1.0064  & -1.0048   & -1.0050    & -0.9993   \\
%B2       & -1.8415  & -1.8414  & -0.8398   & -1.8396    & -1.8406  \\
%B3       & -0.8040  & -0.7934  & -0.7998   & -0.7928    & -0.7868  \\
%\\
% \end{tabular}
%\caption{\label{cap:algo_comp} Performance comparison of estimators for the stacked redshift PDF evaluated using the mean negative log-likelihood loss (Eqn. \ref{eq:snlp}). We compare the Quantile Regression Forest (QRF), ordinal classification PDF estimator (OCP), nonordinal classification PDF estimator (NOCP), ordinal classification PDF estimator with Gaussian mixture model (short GMM) and Highest Weight Element (HWE) (see \S \ref{algorithms}). The SMNLL row denotes the loss derived using the whole dataset, B1, B2 and B3 denote the performance in the respective bins (see text). }
%\end{center}
%\end{table}


%\begin{figure}
%   \centering
% 	\includegraphics[scale=0.4]{./plots_indiv_stack/comparison_distri.pdf}
%   \caption{ \label{comparison_distri} Sample redshift PDF estimated using the ordinal classification PDF estimator (OCP), the ordinal classification PDF estimator with Gaussian mixture model (OCP-GMM), the Highest Weight Element (HWE) and the spectroscopic redshifts.   } 
%\end{figure}


%\\
%The discussion focusses on three main points. Treating the binned redshift as an ordinal attribute as done in the OCP and OCP-GMM algorithms improves the quality of the estimated cond. PDFs. The stacked photometric redshift distribution can be accurately estimated with a single floating point number, the highest weight element (\S \ref{subsec:hwe}).


%Because we evaluate the models in redshift bins (Tab. \ref{subsec:smnlp}), we require a sufficient amount of test data to provide a fair estimate of generalization performance. The validation set is used very frequently in the evaluation process because it is employed to establish appropriate parameters for both the algorithm that estimates the weights in Equation (\ref{eq:cond_prob}) and the kernel density estimate (\S \ref{algorithms}). We therefore traded off computational speed with estimation accuracy of the model error by picking 2800 objects as a suitable data set size for the validation set.
%The training set consisting of 15000 objects is large enough to keep the model variance under control while maintaining computational efficiency.

%\begin{equation}
%	\hat{p}(z | \mathbf{f}) = \sum_{i = 1}^{N_{\rm train}} w_i(\mathbf{f}) K(z, z_{i}^{\rm spec}, h) \, ,
%	\label{eq:cond_pdf_estim}
%\end{equation}

%
%\\
%Our implementation of OCP using the simple bandwidth selection scheme described in \citet{Frank2009} performs well compared with the algorithm employed by \citet{Frank2009} as tested on a subsample of the SDSS Main Galaxy sample \citep{Strauss2002}. 
